Nash Equilibrium in Games on Graphs with Incomplete Preferences

Games with incomplete preferences are an important model for studying rational decision-making in scenarios where players face incomplete information about their preferences and must contend with incomparable outcomes. We study the problem of computing Nash equilibrium in a subclass of two-player games played on graphs where each player seeks to maximally satisfy their (possibly incomplete) preferences over a set of temporal goals. We characterize the Nash equilibrium and prove its existence in scenarios where player preferences are fully aligned, partially aligned, and completely opposite, in terms of the well-known solution concepts of sure winning and Pareto efficiency. When preferences are partially aligned, we derive conditions under which a player needs cooperation and demonstrate that the Nash equilibria depend not only on the preference alignment but also on whether the players need cooperation to achieve a better outcome and whether they are willing to cooperate.We illustrate the theoretical results by solving a mechanism design problem for a drone delivery scenario.

==> sections_dtptb/literature.tex <==
\begin{itemize}
	\item[\textbf{Literature}]
	A stochastic game with preference is different from similar games studied in literature.
	
	\item \textbf{(Normal-form games with preferences).} 
	An important paper on this topic is by Sophie Bade \cite{bade2005nash}. 
	The game considered is $H = \langle (A_i)_{i = 1, \ldots, n}, (\succeq_i)_{i = 1, \ldots, n}\rangle$ where $A_i$ is the set of actions available to player-$i$ and $\succeq_i$ is a preorder on the space of outcomes $\bigtimes_{i = 1, \ldots, n} A_i$.
	The question of interest is to comment on existence and characterization of Nash equilibrium in the game.
	
	\textit{Key ideas/result: }
	\begin{itemize}
		\item Every incomplete preference (preorder) has a completion: Given a (possibly incomplete) preorder $\succeq$ there exists a \emph{complete} preorder $\succeq'$ such that $x \succeq y$ implies $x \succeq' y$ and $x \succ y$ implies $x \succ' y$. 
		
		\item Def. (Completion of game). A game $H'$ is a completion of $H$ if, for all $i \in N$, $\succeq_i'$ is a completion of $\succeq_i$. 
		
		\item Def. (Nash equilibrium). An action profile $a = (a_1, a_2, \ldots, a_n)$ is a Nash equilibrium if, for no player $i$, there exists action $a_i'$ such that $(a_i', a_{-1}) \succ_i (a_i, a_{-1})$. 
		
		\item Given a normal-form game $H$, the set of Nash equilibrium in $H$ is the set
		\begin{align*}
			NE(H) = \bigcup \{NE(H') \mid H' \text{ is a completion of } H\}.
		\end{align*}
	\end{itemize}
	
	\textbf{My Comments.} \emph{I have iterated through all papers on Google Scholar referencing Bade's paper.} 
	
	\begin{itemize}			
		\item The work along with 
		\item The notion of \emph{completion} used by Bade is debatable. 
		The papers \cite{bosi2012continuous,evren2011incomplete} argue that the such a completion exists only when certain separability conditions hold. 
		On the other hand, if the clause ``$x \succ y$ implies $x \succ' y$'' is dropped, the completion $\succ'$ is guaranteed to exist. 
		Hence, Bade's results are restrictive.
		
		\textit{Remark. No other paper fixes this issue.}
		
		\item Since the model is normal-form game, the results carry over to games on graphs. 
	\end{itemize}
	
	
	\item \textbf{(Poset Games).} 
	Poset games \cite{soltys2011complexity,byrnes2002poset} are two-player impartial combinatorial games. 
	(From \cite{byrnes2002poset}) In order to play a poset game, given any poset $A$, two players take turns making moves.
	On each move, a player picks an element $x \in A$, and removes all the elements of $A$ greater than or equal to $x$ from the set $A$, to form a smaller poset $A'$. 
	This becomes the new $A$, then the other player picks an element, and so on. 
	The player unable to move (when $A = \emptyset$) loses. 
	
	\textbf{My Comments}. 
	This game is irrelevant to our setting, unless I'm missing some connection.
	A reduction from stochastic game with preferences to this model is unlikely.
	
	\item \textbf{(Partial Order Games).}
	A partial order game \cite{zahoransky2021partial} is a non-cooperative game model in which players' decision nodes are partially ordered by a dependence relation, which directly captures informational dependencies in the game.
	
	
	\begin{itemize}
		\item \textbf{(Key idea).} 
		PO game is an alternative to extensive form games for expressing a (finite) sequential game. 
		Instead of reasoning with information sets (as used in extensive form games), it asks the user to specify a partial order on decision nodes (think of it as nodes of extensive form game tree). 
		If $x > y$ holds under given partial order, then the decision at $x$ is informed of players' choice at $y$. 
		
		\item PO game model is as expressive as extensive form game with imperfect information, but is exponentially compact to represent. 
		
		\item Every PO game can be represented as a normal form game. 
	\end{itemize}
	
	\textbf{My Comments.} 
	The model is not suitable to study infinite games/games on graphs model. 
	A reduction from stochastic game with preferences to this model is unlikely.
	
	
	\item \textbf{(Posetal Games).} 
	In a posetal game \cite{zanardi2022posetal}, each player expresses a preference over the outcomes via a partially ordered set of metrics.
	The paper proves the existence of pure Nash equilibria. 
	
	\begin{itemize} 
		\item \textbf{(Key idea).} 
		Define a set of real-valued metrics $\calM$, thus, defining a vector of metrics. 
		Now, define a \emph{finite} space of outcomes, \eg, sampled trajectories from a planner. 
		Evaluate metric $m \in \calM$ on every trajectory to rank all trajectories. 
		Select the maximal one.
		
		
		\item \textbf{(Beating around the bush!)} 
		The authors are trying to model combinative preferences, but lack the correct formalism.
		
		\item \textbf{(Not reactive).} 
		The posetal game is a normal-form game. 
		
		Hence, in real scenario, recomputing the entire solution will be required at every time step, which could be tedious.
	\end{itemize}
	
	
	\item \textbf{(Stochastic Games with Lexicographic Objectives)}	 	
	Lexicographic order allows one to consider multiple objectives with a strict preference order.
	We present an algorithm that computes the lexicographically optimal strategies via a reduction to the computation of optimal strategies in a sequence of single-objectives games.
	For omega-regular objectives, we restrict our analysis to one-player games, also known as Markov decision processes.
	We present an algorithm that solves the relevant decision problem in polynomial time.
	
	(Ex.1 from \cite{chatterjee2023stochastic}), consider a lex-objective $\{\mathsf{Reach}(S_1), \mathsf{Safe}(S_2)\}$. 
	Then, a player must first maximize the probability to reach $S_1$ and, moreover, among all optimal strategies for $\mathsf{Reach}(S_1)$, it must choose one that maximizes the probability for $\mathsf{Safe}(S_2)$.
	
	\begin{itemize}
		\item \textbf{(Less general).} 
		\prefltlf model subsumes lexicographic preferences.  
		Also, complexity of solving for \prefltlf is no more than lexicographic preferences. 
		
		\item \textbf{(Not combinative).} 
		\prefltlf ranks strategies by reasoning over satisfying all possible combinations of \ac{ltlf}. 
		Chatterjee's paper does not. 
		
		\item \textbf{(Quantitative).}
		Chatterjee's paper presents quantitative solution along with PRISM integration, which is more appealing. 
	\end{itemize}
	
	
	
	\item \textbf{(Accumulation of Partial Orders).} 
	The accumulation (and aggregation) of partial orders is defined as an algebra in \cite{kiebling2002foundations}. 
	For us, the Pareto accumulation is of interest. 
	Given two orders $\langle \Phi_1, \succeq_1 \rangle$ and $\langle \Phi_2, \succeq_2 \rangle$, the Pareto accumulated order $\langle \Phi_1 \cup \Phi_2, \succeq \rangle$ is given by 
	\begin{align*}
		(x_1, y_1) \succeq (x_2, y_2) \iff 
		(x_1 \succeq_1 x_2 \land \neg (y_2 \succeq_2 y_1)) \lor 
		(y_1 \succeq_2 y_2 \land \neg (x_2 \succeq_1 x_1))
	\end{align*}
	The maximal elements in $\Phi_1 \cup \Phi_2$ under $\succeq$ are Pareto optimal.
	
	A natural question arises that \emph{given a stochastic game $G$, why can we not Pareto accumulate the preferences $\succeq_1$ and $\succeq_2$ of P1 and P2 into $\succeq$, and then find a strategy profile $(\pi_1, \pi_2)$ that achieves a Pareto optimal outcome under $\succeq$?}
	
	For this, we turn to relation between Nash equilibrium and Pareto optimality.
	For normal form games, it is known that NE and Pareto optimality are not equivalent (see example in \url{https://www.quora.com/What-is-the-difference-between-Nash-Equilibrium-and-Pareto-Optimality}). 
	
	In games on graphs, the same non-equivalence holds. 
	In fact, it can be proved that \emph{not all maximal outcomes in Pareto accumulated order are NE.} and \emph{not all NE are maximal in Pareto accumulated order.}
	
	For the first statement, consider a 3 state concurrent game graph where initial state is $s_0$, $T(s_0, (a, c)) = s_1$ and $T(s_0, (b, c)) = s_2$. 
	Suppose that P1 satisfies $\varphi_1$ by visiting $s_1$ and $\varphi_1'$ by visiting $s_2$, and P2 satisfies $\varphi_2$ by visiting $s_1$ and $\varphi_2'$ by visiting $s_2$. 
	Furthermore, let $\varphi_1' \succeq_1 \varphi_1$ and $\varphi_2 \succeq_2 \varphi_2'$. 
	Then, under Pareto accumulation, maximal element is $(\varphi_1', \varphi_2)$. 
	However, it is not realizable in the given game. 
	Among the achievable outcomes, both $(\varphi_1, \varphi_2)$ and $(\varphi_1', \varphi_2')$ are maximal. 
	However, only $(\varphi_1', \varphi_2')$ is a NE. 
	Thus, the achievable maximal outcome $(\varphi_1, \varphi_2)$ is not a NE.
	
	A similar game may be constructed to prove the second statement.
	Try to show that $(\emptyset, \emptyset)$ is a NE, but not maximal.
	
	
	\textbf{My Comment.} The above propositions highlight that, in stochastic games with preferences, realizability of \ac{ltlf} alternatives plays a key role. 
	We must reason about \emph{maximal realizable outcomes} to identify the NE in these interactions.		
\end{itemize}



\aknote{Coalition games}

\ak{Based on my skimming (as of 12 April), it is reasonable to assume that stochastic games with preference as we define are not studied. Or, even if studied, the solution approach we propose is not explored. }

We need to deep dive into Coalition games, Coalition logic literature to show how our approach may address existing shortcomings in these areas! 


==> sections_dtptb/nash.tex <==
%\aknote{Answer the following questions in this section.
%
%1. What are existing notions of Nash equilibrium from literature? Do they apply to our setting? If yes, great! If not, why not?
%
%2. Define maximal distributions / stochastic order.
%
%3. Define Nash equilibrium in terms of maximal distributions, not maximal paths determined by strategy profile.
%
%4. Does there exist a NE in stochastic game with preferences?
%
%5. Is NE unique?
%
%6. Is NE a good equilibrium concept to analyze stochastic games with preferences?
%}


In this section, we formalize the notion of Nash equilibrium in a stochastic game with preference $G$.


Recall that a strategy profile $(\pi_1, \pi_2)$ induces a probability distribution over the set of paths, which we denote by $\mathsf{Pr}^{\pi_1, \pi_2}$.
Then, following \cite{bade2005nash}, we informally define Nash equilibrium in $G$ as follows:

\begin{mdframed}[roundcorner=10pt]
	A strategy profile $(\pi_1^*, \pi_2^*)$ is NE in $G$ if and only if

	(a) There exists no strategy $\pi_1 \in \Pi_1$ such that $\mathsf{Pr}^{\pi_1, \pi_2^*}$ is \emph{strictly preferred to} $\mathsf{Pr}^{\pi_1^*, \pi_2^*}$; and

	(b) There exists no strategy $\pi_2 \in \Pi_2$ such that $\mathsf{Pr}^{\pi_1^*, \pi_2}$ is \emph{strictly preferred to} $\mathsf{Pr}^{\pi_1^*, \pi_2^*}$.
\end{mdframed}


To formalize this notion, we need a way to compare two probability distributions under a preference relation.
For this, we turn to the theory of stochastic orders \cite{massey1987stochastic}.
A stochastic order quantifies the concept of one random variable being ``greater'' than another.


Given a finite preference model $(U, \geq)$, let $\familyI(U)$ be a family of subsets of $U$ that includes $U$ itself and the empty set.
Given two probability distributions $P_1$ and $P_2$ over $U$, we say that $P_1 \geq_\familyI P_2$ whenever $P_1(X) \geq P_2(X)$ for all $X \in \familyI(U)$.


\begin{definition}[{\cite[Def. 2.1]{massey1987stochastic}}]
	\label{def:stochastic-ordering}
	The ordering $\geq_\familyI$ is a \emph{stochastic ordering} on $U$ if
	\begin{enumerate}[i.]
		\item The relation $\geq_\familyI$ is a partial order on the space of probability measures.
		\item Let $\delta_u$ be the point mass measure on $U$ for some $u \in U$. For all $u, v \in U$, $u \geq v$ if and only if $\delta_u \geq_\familyI \delta_v$.
	\end{enumerate}
\end{definition}


Def.~\ref{def:stochastic-ordering} specify the necessary conditions on family $\familyI(U)$ of subsets of $U$ and the order $\geq_\familyI$ required to define a stochastic order.
Condition (i) states that $\familyI(U)$ should be constructed using a \emph{determining class} \cite{obrien1982determining}, \ie, a set of functions using which we can recover the probability distribution $P$ on $U$ given the measure on $\familyI(U)$.


\begin{example}
	Suppose that $U = \{u_1, u_2, u_3, u_4\}$ and $\geq = \{(u_1, u_2), (u_1, u_3), (u_2, u_4), (u_3, u_4)\}$.
	Then, the set $\{\emptyset, \{u_1\}, \{u_1, u_2\}, \{u_1, u_3\}, U\}$ is a valid family of subsets.
	Here, if the probability distribution on $U$ is defined as $P(u_1) = 0.1$, $P(u_2) = 0.2$, $P(u_3) = 0.3$, and $P(u_4) = 0.4$, then a measure $Q$ on $U$ can be defined as $Q(\emptyset) = 0$, $Q(\{u_1\}) = 0.1$, $Q(\{u_1, u_2\}) = 0.3$, $Q(\{u_1, u_3\}) = 0.4$, and $Q(U) = 1$.
	Notice that the distribution $P$ can be recovered from $Q$.
\end{example}


Condition (ii) states the required properties that family of subsets $I(U)$ must satisfy.
These are the same as those required for the existence of a multi-utility representation \cite{ok2002utility,evren2011incomplete}.

The statement $\delta_u \geq_I \delta_v$ is interpreted as follows: Given a family of subset $[\emptyset, U_1, U_2, \ldots, U_n, U]$, $\delta_x$ is a boolean vector $[0, x \in U_1, x \in U_2, \ldots, x \in U_N, 1]$.
Thus, $x \geq y$ if and only if the vector $\delta_x$ is greater than or equal to the vector $\delta_y$.

\begin{example}
	Let us continue with the previous example.
	Given a family of subset $\{\emptyset, \{u_1\}, \{u_1, u_2\}, \{u_1, u_3\}, U\}$, $\delta_{u_2}$ is a boolean vector $[u_2 \in X \mid X \in \familyI(U)] = [0, 0, 1, 0, 1]$.
	Similarly, $\delta_{u_4}$ is a boolean vector $[0, 0, 0, 0, 1]$.
	Then, condition (ii) requires that if $u_2 \geq u_4$ then $\delta_{u_2} \geq \delta_{u_4}$..
	Since the conditions (i) and (ii) are satisfied by our choice of $\familyI(U)$ and $\geq_\familyI$ on $U$, $\geq_\familyI$ is a valid stochastic order on $U$.
\end{example}


Massey \cite{massey1987stochastic} provides a characterization of stochastic orders.
We need two definitions to understand the result.
Given a partial order $\geq$ on $U$, a subset $X$ of $U$ is called an \emph{increasing set} if $X = \{y \in U \mid y \geq x \text{ for some } x \in X\}$.
A family of subsets $\familyI(U)$ is called \emph{strongly separating} if for all $v \not\geq u$, there exists a subset $X \in \familyI(U)$ such that $u \in X$ and $v \notin X$.
It is noted that condition (i) in Def.~\ref{def:stochastic-ordering} is always satisfied whenever $U$ is finite and $\familyI(U)$ is strongly separating.


\begin{proposition}
	$\familyI(U)$ induces a stochastic order on $U$ if and only $\familyI(U)$ is a strongly separating family of increasing sets that form a determining class.
\end{proposition}



\begin{remark}
	It is important to note that Massey's results apply to \emph{partial orders} on countable (infinite) sets $U$.
	This is not the case in our paper.
	I have tried to adopt/simplify Massey's results in our context.
\end{remark}


Massey \cite{massey1987stochastic} introduced three stochastic orders.

\begin{definition}
	Let $\familyI_{st}(U)$, $\familyI_{wk}(U)$, and $\familyI_{wk*}(U)$ denote the strong, weak, and weak* orderings, respectively.
	It is defined that
	\begin{align}
		\familyI_{st}(U) = \{\text{ all increasing sets in $2^U$} \} \\
		\familyI_{wk}(U) = \{\{x\}^\uparrow \mid x\in U \} \cup \{U, \emptyset\}  \\
		\familyI_{wk*}(U) = \{E\setminus \{x\}^\downarrow \mid x\in U \} \cup \{U, \emptyset\}
	\end{align}
\end{definition}

These stochastic orderings allow us to rank probability measures according to the partially ordered set $U$.
%
Let $\familyI(U)$ be \emph{a family of subsets} of $U$ that includes $U$ itself and the empty set $\emptyset$. That is, $\familyI \in \{\familyI_{st}, \familyI_{wk}, \familyI_{wk*}\}$.
%
Let $P_1$ and $P_2$ be two probability measures on $U$. We denote $P_2\ge_{\familyI}P_1$
whenever $P_2(X) \ge_{\familyI} P_1(X)$ for all subsets $X\in \familyI(U)$.
It is proven that if the partial order $U$ is a total order, then the three stochastic orderings $\familyI_{st}(U)$, $\familyI_{wk}(U)$, and $\familyI_{wk*}(U)$  are equivalent \cite[Prop.~2.5]{massey1987stochastic}.
However, for a partial order, the three stochastic orderings may differ.


%\begin{example}[{\cite{rahmani2024preference}}]
%	Let $U = \{a,b,c,d\}$ and  $\succeq = \{(a, b), (b, d), (c, d), (a, c), (a, d) \} \cup I_U$, where $I_U$ is the identity relation on $U$ and that $(x,y)\in \succeq$ if and only if $x\succeq y$.
%	%
%	Also, consider probability measures $P_1$, $P_2$, and $P_3$ where $P_1(a)=0.5, P_1(b)=0.3, P_1(c)=0.2$, $P_2(b) = 0.5, P_2(c) = 0.3, P_2(d) = 0.2$, and $P_3(a) = 0.3, P_3(b) = 0.2, P_3(d) = 0.5$.
%	%
%
%	We have
%	\[
%		\familyI_{st}(U) = \{ \{a\}, \{a,b\}, \{a,c\}, \{a, b, c \}, \{a,b,c,d\}, \emptyset\}.
%	\]
%	%
%	Accordingly,
%	\[
%	[P_1[X]]_{X\in	\familyI_{st}(U) }= [0.5, 0.8, 0.7, 1, 1, 0],
%	\]
%	\vspace{-18pt}
%	\[
%	[P_2[X]]_{X\in	\familyI_{st}(U) }= [0, 0.5, 0.3, 1, 1, 0], \text{and}
%	\]
%	\vspace{-18pt}
%	\[
%	[P_3[X]]_{X\in 	\familyI_{st}(U) }   = [0.3, 0.5, 0.3, 0.5, 1, 0].
%	\]
%	%
%	Therefore, $P_1 >_{\familyI_{st}} P_2$, $P_1 >_{\familyI_{st}} P_3$. None of $P_2$ and $P_3$ strong-stochastic dominates the other one.
%
%	Also, we have
%	\[
%	\familyI_{wk}(U) = \{ \{a\}, \{a,b\}, \{a,c\}, \{a,b,c,d\}, \emptyset\}.
%	\]
%	%
%
%	%
%	Accordingly,
%	\[
%	[P_1[X]]_{X\in	\familyI_{wk}(U) }= [0.5, 0.8, 0.7, 1, 0],
%	\]
%	\vspace{-18pt}
%	\[
%	[P_2[X]]_{X\in	\familyI_{wk}(U) }= [0, 0.5, 0.3, 1, 0], \text{and}
%	\]
%	\vspace{-18pt}
%	\[
%	[P_3[X]]_{X\in 	\familyI_{wk}(U) }   = [0.3, 0.5, 0.3, 1, 0].
%	\]
%	%
%	Thus, $P_1 >_{\familyI_{wk}} P_2$, $P_1 >_{\familyI_{wk}} P_3$, and $P_3 >_{\familyI_{wk}} P_2$.
%	%
%
%	Also, we have
%	\[
%	\familyI_{wk*}(U) = \{ \{a,b\}, \{a,c\}, \{a, b, c \}, \{a,b,c,d\}, \emptyset\}.
%	\]
%	%
%
%	%
%	Accordingly,
%	\[
%	[P_1[X]]_{X\in	\familyI_{wk*}(U) }= [0.8, 0.7, 1, 1, 0],
%	\]
%	\vspace{-18pt}
%	\[
%	[P_2[X]]_{X\in	\familyI_{wk*}(U) }= [0.5, 0.3, 0.8, 1, 0], \text{and}
%	\]
%	\vspace{-18pt}
%	\[
%	[P_3[X]]_{X\in 	\familyI_{wk*}(U) }   = [0.5, 0.3, 0.5, 1, 0].
%	\]
%	%
%	Thus, $P_1 >_{\familyI_{wk*}} P_2$, $P_1 >_{\familyI_{wk*}} P_3$, and $P_2 >_{\familyI_{wk*}} P_3$.
%	%
%\end{example}



\aknote{
	The fundamental understanding about the properties of $\familyI$ can enable us to define other stochastic orders. For instance, an order that values satisfying more number of \ac{ltlf} formulas or a lexicographic order (if possible!).

	In general, I think it will suffice to prove that family of subsets is separating and, therefore, defines a determining class along with condition (ii).

	For now (on 15 April), I'll stop here.
}



\subsection{Formalizing Nash Equilibrium}

\begin{definition}
	\label{def:sto_dominance}
	%	
	Given a stochastic game with preferences $\langle G, \Phi, \psi_1, \psi_2 \rangle$, let $\langle \Phi, \weakpref_1 \rangle$ and $\langle \Phi, \weakpref_2 \rangle$ be the preference models induced by $\psi_1$ and $\psi_2$, respectively.
	A strategy profile $(\pi_1^*, \pi_2^*)$ is \emph{$\familyI$-stochastic undominated}
	with respect to P1 if there \emph{does not exist} any P1 strategy $\pi_1$ such that $\mathsf{Pr}^{\pi_1, \pi_2^*} \geq_\familyI \mathsf{Pr}^{\pi_1^*, \pi_2^*}$.
\end{definition}


\begin{definition}
	\label{def:nash-equilibrium}
	%	
	A strategy profile $(\pi_1^*, \pi_2^*)$ is a NE in $\calG$ if and only if it is $\familyI$-stochastic undominated for P1 and P2.
\end{definition}


Next, we ask whether the NE is unique? Not surprisingly, it is not. 

\begin{proposition}
	NE in $\calG$ may not be unique. 
\end{proposition}
\begin{proof}[Proof (Idea)]
	Consider a game $G$ with states $\{s_0, \ldots, s_4\}$, where $s_0$ is an initial state and each player has two possible actions $\{a, b\}$. The transitions are given as follows: $T(s_0, (a, a)) = s_1, T(s_0, (a, b)) = s_2, T(s_0, (b, a)) = s_3, T(s_0, (b, b)) = s_4$. Suppose that both P1 and P2 prefer $s_1$ to $s_2, s_3$ and $s_4$ to $s_2, s_3$. 
	
	Here, we have two NE: $\pi_1(s_0) = \{a\}, \pi_2(s_0) = \{a\}$ and $\pi_1'(s_0) = \{b\}, \pi_2'(s_0) = \{b\}$. 
\end{proof}

Note that the above game can also modeled as a matrix game. 


\ak{What about existence of NE?}

For the example in \url{https://youtu.be/8Q2XbllUSLc}, there is no Nash equilibrium in matrix form. 
However, under our definition of $\familyI_{wk}$-stochastic undomination LH is a NE. 

\ak{Write this example! This is insightful to anyone familiar with normal form games! Check if it has NE under wk-star and strong order.}


\aknote{
	I'm unable to find an attack vector on proving/disproving existence of NE.
	
	1. For stochastic games (Chatterjee) shows NE does not exist for single objective. But $\epsilon$-NE always exists for all $\epsilon > 0$. 
	
	2. Explore literature on multi-objective stochastic games (de Alfaro, Kwiatkowska, Chatterjee's work). 
	
	3. My hunch is that NE or $\epsilon$-NE must exist for SGwP. This should relate somehow to value determinacy of stochastic games with single objectives and $\familyI(U)$. 
} 

\ak{On 17 Apr. I decide to revisit existence problem after design of synthesis solution.}

\aknote{Another idea could be to look at qualitative determinacy, and reason about almost-surely winnable objectives. This will allow us to exploit the idea of improvement!}
